RelitLRM: Generative Relightable Radiance for Large Reconstruction Models

We propose RelitLRM, a Large Reconstruction Model (LRM) for generating high-quality Gaussian splatting representations of 3D objects under novel illuminations from sparse (4-8) posed images captured under unknown static lighting. Unlike prior inverse rendering methods requiring dense captures and slow optimization, often causing artifacts like incorrect highlights or shadow baking, RelitLRM adopts a feed-forward transformer-based model with a novel combination of a geometry reconstructor and a relightable appearance generator based on diffusion. The model is trained end-to-end on synthetic multi-view renderings of objects under varying known illuminations. This architecture design enables to effectively decompose geometry and appearance, resolve the ambiguity between material and lighting, and capture the multi-modal distribution of shadows and specularity in the relit appearance. We show our sparse-view feed-forward RelitLRM offers competitive relighting results to state-of-the-art dense-view optimization-based baselines while being significantly faster. Our project page is available at: https://relit-lrm.github.io/.

==> tables/tbl_exp_deterministic.tex <==
\begin{table}[t]
    \centering
    % \scriptsize
    \fontsize{7.5pt}{11pt}\selectfont
    \caption{ \textbf{Ablation on probabilistic design}. We design a deterministic counterpart by removing the noisy image tokens and keep the model architecture and training configuration the same. We compare our probabilistic design with the deterministic counterpart on our holdout evaluation set. 
    % \TYZ{Might remove the last two rows of 8 input views. The point we use diffusion is not to get  a higher PSNR, is that we can render specular objects much better.  }
    }
    \label{tbl:exp_determin}
    \begin{tabular}{lcccc}
    \toprule
          &  Input Views & PSNR & SSIM & LPIPS   \\
      \midrule
      Ours-Probabilistic & 4 & 27.63  & 0.922& 0.064   \\
      \midrule
      Ours-Deterministic & 4 & 27.10  & 0.912 & 0.076   \\
      \midrule
    \bottomrule
      % Ours over Single view & 81.0\% & 86.0\%
    \end{tabular}
    % \aftertab
\end{table}


 % Ours-Probabilistic & 8 & 29.45 & 0.937 & 0.052   \\
 %      \midrule
 %      Ours-Deterministic & 8 &  & &   \\

==> tables/tbl_exp_img.tex <==
\begin{table}[t]
    \centering
    % \scriptsize
    \fontsize{7.5pt}{11pt}\selectfont
    \caption{\textbf{Compare with image-based relighting models on hold-out validation set.} The prediction is scaled per-channel to align with target following~\citep{jin2024gaffer}. The PSNR is only computed in masked foreground regions. Our methods takes four input views, and baseline methods take each view independently. }
    \label{tbl:exp_img}
    \begin{tabular}{lccccc}
    \toprule
          & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & NFE & Parameters  \\
      \midrule
      Ours &  \textbf{28.50} &\textbf{ 0.93} & \textbf{0.058} &  5 & 0.4B \\
      NeuralGaffer & 24.51 & 0.90 & 0.072 & 50  & 0.9B \\
      \midrule
      DiLightNet & 20.02  & 0.85 &  0.132 & 20 & 0.9B \\
    \bottomrule
      % Ours over Single view & 81.0\% & 86.0\%
    \end{tabular}
    % \aftertab
\end{table}

